A practical algorithm for 2-admissibility

The $2$-admissibility of a graph is a promising measure to identify real-world networks which have an algorithmically favourable structure. In contrast to other related measures, like the weak/strong $2$-colouring numbers or the maximum density of graphs that appear as $1$-subdivisions, the $2$-admissibility can be computed in polynomial time. However, so far these results are theoretical only and no practical implementation to compute the $2$-admissibility exists. Here we present an algorithm which decides whether the $2$-admissibility of an input graph $G$ is at most $p$ in time $O(p^4 |V(G)|)$ and space $O(|E(G)| + p^2)$. The simple structure of the algorithm makes it easy to implement. We evaluate our implementation on a corpus of 214 real-world networks and find that the algorithm runs efficiently even on networks with millions of edges, that it has a low memory footprint, and that indeed many networks have a small $2$-admissibility.

==> figures/table.tex <==
\begin{longtable}{lrrrrrrrrr}
Network & $\adm_2$ & $\bar d$ & $\text{deg}$ & $\Delta$ & $m$ & $n$ & Load(kb) & Usage(kb) & Time(s) \\
\hline
AS-oregon-1 & 28 & 4.19 & 17 & 2389 & 23409 & 11174 & 1560.89 & 5343.72 & 0.48 \\
AS-oregon-2 & 52 & 5.71 & 31 & 2432 & 32730 & 11461 & 1642.18 & 5593.12 & 1.00 \\
BioGrid-Affinity-Capture-Luminescence & 8 & 2.51 & 6 & 376 & 2312 & 1840 & 445.20 & 1252.80 & 0.07 \\
BioGrid-Affinity-Capture-Ms & 183 & 15.90 & 58 & 2217 & 321887 & 40495 & 9174.07 & 33281.05 & 72.31 \\
BioGrid-Affinity-Capture-Rna & 75 & 6.22 & 54 & 3572 & 42815 & 13765 & 1837.80 & 6239.51 & 1.09 \\
BioGrid-Affinity-Capture-Western & 64 & 6.09 & 17 & 535 & 64046 & 21028 & 3158.82 & 11368.61 & 3.11 \\
BioGrid-All & 476 & 34.86 & 131 & 3620 & 1316843 & 75550 & 28946.62 & 103501.16 & 883.84 \\
BioGrid-Arabidopsis-Thaliana-Columbia & 53 & 9.20 & 26 & 1341 & 47916 & 10417 & 1845.78 & 6512.89 & 2.85 \\
BioGrid-Biochemical-Activity & 29 & 4.12 & 11 & 427 & 17746 & 8620 & 1572.68 & 5211.81 & 0.45 \\
BioGrid-Bos-Taurus & 4 & 1.87 & 3 & 27 & 424 & 454 & 170.70 & 308.45 & 0.03 \\
BioGrid-Caenorhabditis-Elegans & 70 & 7.40 & 64 & 522 & 23646 & 6394 & 978.66 & 3335.76 & 0.78 \\
BioGrid-Candida-Albicans-Sc5314 & 9 & 2.87 & 9 & 427 & 1609 & 1121 & 265.64 & 637.82 & 0.06 \\
BioGrid-Canis-Familiaris & 2 & 1.75 & 2 & 90 & 125 & 143 & 105.33 & 105.33 & 0.02 \\
BioGrid-Chemicals & 1 & 1.69 & 1 & 413 & 28093 & 33266 & 5449.23 & 19875.67 & 0.51 \\
BioGrid-Co-Crystal-Structure & 5 & 1.76 & 5 & 92 & 2021 & 2291 & 432.72 & 1246.29 & 0.08 \\
BioGrid-Co-Fractionation & 83 & 10.23 & 83 & 187 & 56354 & 11017 & 1978.86 & 6922.47 & 2.38 \\
BioGrid-Co-Localization & 9 & 2.51 & 6 & 63 & 4452 & 3543 & 443.30 & 1316.80 & 0.09 \\
BioGrid-Co-Purification & 12 & 2.76 & 12 & 1972 & 5970 & 4326 & 808.07 & 2552.52 & 0.21 \\
BioGrid-Cricetulus-Griseus & 1 & 1.65 & 1 & 30 & 57 & 69 & 93.68 & 93.68 & 0.02 \\
BioGrid-Danio-Rerio & 3 & 2.04 & 3 & 61 & 266 & 261 & 127.07 & 157.44 & 0.02 \\
BioGrid-Dictyostelium-Discoideum-Ax4 & 1 & 1.48 & 1 & 4 & 20 & 27 & 85.73 & 85.73 & 0.03 \\
BioGrid-Dosage-Growth-Defect & 9 & 3.03 & 5 & 213 & 2193 & 1447 & 261.90 & 652.36 & 0.04 \\
BioGrid-Dosage-Lethality & 8 & 2.58 & 4 & 392 & 2289 & 1776 & 261.92 & 663.84 & 0.04 \\
BioGrid-Dosage-Rescue & 11 & 3.81 & 7 & 75 & 6444 & 3380 & 453.51 & 1385.21 & 0.10 \\
BioGrid-Drosophila-Melanogaster & 83 & 12.98 & 83 & 303 & 60556 & 9330 & 2003.70 & 7080.36 & 3.98 \\
BioGrid-Emericella-Nidulans-Fgsc-A4 & 2 & 1.94 & 2 & 44 & 62 & 64 & 94.28 & 94.28 & 0.02 \\
BioGrid-Escherichia-Coli-K12-Mg1655 & 10 & 2.97 & 5 & 58 & 1889 & 1273 & 262.50 & 644.16 & 0.07 \\
BioGrid-Escherichia-Coli-K12-W3110 & 290 & 89.40 & 131 & 1187 & 181620 & 4063 & 3859.89 & 12557.59 & 90.82 \\
BioGrid-Far-Western & 3 & 1.82 & 3 & 60 & 1089 & 1199 & 258.45 & 626.99 & 0.03 \\
BioGrid-Fret & 24 & 2.82 & 19 & 51 & 2395 & 1700 & 259.59 & 662.16 & 0.08 \\
BioGrid-Gallus-Gallus & 4 & 2.11 & 4 & 110 & 436 & 413 & 126.99 & 162.87 & 0.02 \\
BioGrid-Glycine-Max & 2 & 1.77 & 2 & 13 & 39 & 44 & 88.31 & 88.31 & 0.03 \\
BioGrid-Hepatitus-C-Virus & 1 & 1.97 & 1 & 133 & 134 & 136 & 105.31 & 105.31 & 0.03 \\
BioGrid-Homo-Sapiens & 263 & 30.69 & 71 & 2882 & 369767 & 24093 & 9625.87 & 30177.38 & 92.36 \\
BioGrid-Human-Herpesvirus-1 & 3 & 2.34 & 3 & 40 & 208 & 178 & 105.47 & 105.47 & 0.03 \\
BioGrid-Human-Herpesvirus-4 & 2 & 2.02 & 2 & 154 & 326 & 323 & 127.41 & 161.15 & 0.03 \\
BioGrid-Human-Herpesvirus-5 & 1 & 1.77 & 1 & 27 & 107 & 121 & 105.18 & 105.18 & 0.02 \\
BioGrid-Human-Herpesvirus-8 & 3 & 1.93 & 3 & 119 & 691 & 716 & 171.72 & 323.39 & 0.04 \\
BioGrid-Human-Immunodeficiency-Virus-1 & 6 & 2.32 & 3 & 324 & 1319 & 1138 & 264.01 & 635.14 & 0.03 \\
BioGrid-Human-Immunodeficiency-Virus-2 & 1 & 1.58 & 1 & 6 & 15 & 19 & 85.88 & 85.88 & 0.05 \\
BioGrid-Human-Papillomavirus-16 & 2 & 2.15 & 2 & 93 & 186 & 173 & 105.64 & 105.64 & 0.04 \\
Cannes2013 & 114 & 3.82 & 27 & 15169 & 835892 & 438089 & 48981.02 & 175852.25 & 230.83 \\
CoW-interstate & 7 & 3.51 & 4 & 25 & 319 & 182 & 104.51 & 104.51 & 0.02 \\
DNC-emails & 28 & 4.70 & 17 & 402 & 4384 & 1866 & 470.83 & 1309.34 & 0.06 \\
EU-email-core & 74 & 32.58 & 34 & 345 & 16064 & 986 & 455.46 & 1376.51 & 1.16 \\
JDK\_dependency & 76 & 16.68 & 65 & 5923 & 53658 & 6434 & 1408.96 & 4554.62 & 1.86 \\
JUNG-javax & 76 & 16.43 & 65 & 5655 & 50290 & 6120 & 1356.07 & 4426.94 & 1.91 \\
NYClimateMarch2014 & 161 & 6.39 & 34 & 14687 & 327080 & 102378 & 13919.95 & 49241.35 & 67.52 \\
NZ\_legal & 68 & 14.70 & 25 & 429 & 15739 & 2141 & 568.23 & 1808.36 & 0.71 \\
Noordin-terror-loc & 4 & 2.99 & 3 & 18 & 190 & 127 & 105.60 & 105.60 & 0.02 \\
Noordin-terror-orgas & 3 & 2.81 & 3 & 21 & 181 & 129 & 105.41 & 105.41 & 0.07 \\
Noordin-terror-relation & 11 & 7.17 & 11 & 28 & 251 & 70 & 94.34 & 94.34 & 0.05 \\
ODLIS & 38 & 11.29 & 12 & 592 & 16377 & 2900 & 590.77 & 1871.51 & 0.36 \\
Opsahl-forum & 42 & 15.65 & 14 & 128 & 7036 & 899 & 348.74 & 857.88 & 0.18 \\
Opsahl-socnet & 61 & 14.57 & 20 & 255 & 13838 & 1899 & 600.60 & 1717.02 & 0.57 \\
StackOverflow-tags & 6 & 4.26 & 6 & 16 & 245 & 115 & 106.36 & 106.36 & 0.07 \\
Y2H\_union & 7 & 2.75 & 4 & 89 & 2705 & 1966 & 423.44 & 1254.80 & 0.08 \\
Yeast & 18 & 6.08 & 6 & 66 & 7182 & 2361 & 481.72 & 1361.24 & 0.13 \\
actor\_movies & 105 & 5.75 & 14 & 646 & 1470404 & 511463 & 103718.56 & 343790.00 & 390.95 \\
advogato & 86 & 15.24 & 25 & 803 & 39285 & 5155 & 1197.26 & 4099.85 & 2.76 \\
airlines & 18 & 11.04 & 13 & 130 & 1297 & 235 & 139.46 & 185.44 & 0.03 \\
american\_revolution & 3 & 2.27 & 3 & 59 & 160 & 141 & 105.50 & 105.50 & 0.03 \\
as-22july06 & 44 & 4.22 & 25 & 2390 & 48436 & 22963 & 3127.22 & 10761.58 & 1.64 \\
as-skitter & 365 & 13.08 & 111 & 35455 & 11095298 & 1696415 & 308145.47 & 1090595.10 & 10768.63 \\
as20000102 & 21 & 3.88 & 12 & 1458 & 12572 & 6474 & 826.55 & 2692.73 & 0.28 \\
autobahn & 3 & 2.56 & 2 & 5 & 478 & 374 & 126.98 & 161.48 & 0.02 \\
bahamas & 8 & 2.24 & 6 & 14902 & 246291 & 219856 & 22366.36 & 84164.58 & 16.98 \\
bergen & 12 & 10.26 & 9 & 32 & 272 & 53 & 91.24 & 91.24 & 0.02 \\
bitcoin-otc-negative & 21 & 4.06 & 16 & 227 & 3259 & 1606 & 270.60 & 695.44 & 0.06 \\
bitcoin-otc-positive & 50 & 6.67 & 20 & 788 & 18591 & 5573 & 889.74 & 2973.39 & 0.70 \\
bn-fly-drosophila\_medulla\_1 & 44 & 10.01 & 18 & 927 & 8911 & 1781 & 360.61 & 1008.70 & 0.29 \\
bn-mouse\_retina\_1 & 223 & 168.79 & 121 & 744 & 90811 & 1076 & 1957.90 & 5630.18 & 8.61 \\
boards\_gender\_1m & 25 & 9.67 & 25 & 88 & 19993 & 4134 & 952.19 & 2885.06 & 0.63 \\
boards\_gender\_2m & 7 & 2.65 & 4 & 45 & 5598 & 4220 & 809.88 & 2534.69 & 0.08 \\
ca-CondMat & 30 & 8.08 & 25 & 279 & 93439 & 23133 & 3535.77 & 12682.73 & 3.19 \\
ca-GrQc & 43 & 5.53 & 43 & 81 & 14484 & 5241 & 872.88 & 2732.29 & 0.25 \\
ca-HepPh & 238 & 19.74 & 131 & 491 & 118489 & 12006 & 2996.30 & 10104.79 & 12.58 \\
capitalist & 21 & 15.41 & 19 & 91 & 1071 & 139 & 114.86 & 120.71 & 0.04 \\
celegans & 21 & 14.46 & 10 & 134 & 2148 & 297 & 146.60 & 239.56 & 0.05 \\
chess & 88 & 15.31 & 29 & 181 & 55899 & 7301 & 2210.87 & 6781.29 & 4.04 \\
chicago & 1 & 1.77 & 1 & 12 & 1298 & 1467 & 260.24 & 639.14 & 0.03 \\
cit-HepPh & 89 & 24.37 & 30 & 846 & 420877 & 34546 & 10494.86 & 37981.65 & 48.77 \\
cit-HepTh & 128 & 25.37 & 37 & 2468 & 352285 & 27769 & 7700.24 & 27419.55 & 51.60 \\
codeminer & 5 & 2.80 & 4 & 55 & 1015 & 724 & 171.79 & 324.96 & 0.06 \\
columbia-mobility & 9 & 9.61 & 9 & 228 & 4147 & 863 & 211.37 & 441.44 & 0.05 \\
columbia-social & 19 & 17.90 & 18 & 545 & 7724 & 863 & 267.89 & 616.05 & 0.09 \\
cora\_citation & 30 & 7.70 & 13 & 377 & 89157 & 23166 & 3480.62 & 12701.12 & 3.76 \\
countries & 16 & 2.11 & 6 & 110602 & 624402 & 592414 & 92037.16 & 325340.25 & 155.42 \\
cpan-authors & 17 & 5.03 & 9 & 327 & 2112 & 839 & 184.45 & 361.74 & 0.05 \\
deezer & 60 & 18.26 & 21 & 420 & 498202 & 54573 & 12043.83 & 43563.95 & 43.88 \\
digg & 46 & 5.68 & 8 & 285 & 86312 & 30398 & 6488.16 & 21257.37 & 5.19 \\
diseasome & 11 & 3.86 & 11 & 84 & 2738 & 1419 & 267.06 & 662.72 & 0.16 \\
dogster\_friendships & 1016 & 40.05 & 131 & 46505 & 8546581 & 426820 & 194447.22 & 624314.94 & 27739.26 \\
dolphins & 6 & 5.13 & 4 & 12 & 159 & 62 & 94.85 & 94.85 & 0.03 \\
dutch-textiles & 5 & 3.75 & 5 & 31 & 90 & 48 & 88.75 & 88.75 & 0.06 \\
ecoli-transcript & 5 & 2.73 & 3 & 74 & 578 & 423 & 127.63 & 165.20 & 0.04 \\
edinburgh\_associative\_thesaurus & 197 & 25.69 & 34 & 1062 & 297094 & 23132 & 6780.44 & 24529.89 & 65.53 \\
email-Enron & 145 & 10.02 & 43 & 1383 & 183831 & 36692 & 7480.81 & 24888.59 & 25.06 \\
escorts & 45 & 4.67 & 11 & 305 & 39044 & 16730 & 3208.14 & 10530.04 & 2.19 \\
euroroad & 3 & 2.41 & 2 & 10 & 1417 & 1174 & 258.82 & 625.63 & 0.07 \\
eva-corporate & 4 & 1.85 & 3 & 552 & 6711 & 7253 & 1432.23 & 4950.11 & 0.11 \\
exnet-water & 3 & 2.55 & 2 & 10 & 2416 & 1893 & 433.43 & 1231.98 & 0.05 \\
facebook-links & 191 & 25.64 & 52 & 1098 & 817090 & 63731 & 20580.54 & 74939.01 & 188.07 \\
foldoc & 36 & 13.70 & 12 & 728 & 91471 & 13356 & 2506.90 & 9015.71 & 3.25 \\
foodweb-caribbean & 23 & 13.47 & 13 & 196 & 3313 & 492 & 201.50 & 397.60 & 0.08 \\
foodweb-otago & 23 & 11.80 & 14 & 45 & 832 & 141 & 112.90 & 113.57 & 0.03 \\
football & 11 & 10.66 & 8 & 12 & 613 & 115 & 108.00 & 108.00 & 0.05 \\
google+ & 38 & 3.32 & 12 & 2761 & 39194 & 23628 & 3099.64 & 10679.88 & 1.11 \\
gowalla & 202 & 9.67 & 51 & 14730 & 950327 & 196591 & 31640.44 & 116517.97 & 180.06 \\
haggle & 40 & 15.50 & 39 & 101 & 2124 & 274 & 148.30 & 239.14 & 0.04 \\
hex & 4 & 5.62 & 3 & 6 & 930 & 331 & 130.15 & 167.64 & 0.03 \\
hypertext\_2009 & 43 & 38.87 & 28 & 98 & 2196 & 113 & 132.26 & 173.63 & 0.06 \\
ia-email-univ & 21 & 9.62 & 11 & 71 & 5451 & 1133 & 293.13 & 762.10 & 0.09 \\
ia-infect-dublin & 21 & 13.49 & 17 & 50 & 2765 & 410 & 157.06 & 276.06 & 0.08 \\
ia-reality & 12 & 2.26 & 5 & 261 & 7680 & 6809 & 803.31 & 2635.98 & 0.25 \\
infectious & 21 & 13.49 & 17 & 50 & 2765 & 410 & 157.04 & 274.55 & 0.06 \\
ingredients & 475 & 197.46 & 133 & 3426 & 431654 & 4372 & 10230.61 & 27386.90 & 97.07 \\
iscas89-s1196 & 4 & 2.85 & 2 & 16 & 537 & 377 & 127.80 & 162.96 & 0.03 \\
iscas89-s1238 & 5 & 3.00 & 2 & 18 & 625 & 416 & 127.98 & 167.24 & 0.02 \\
iscas89-s13207 & 6 & 2.73 & 4 & 37 & 3406 & 2492 & 440.71 & 1273.01 & 0.05 \\
iscas89-s1423 & 3 & 2.62 & 2 & 17 & 554 & 423 & 127.24 & 163.58 & 0.03 \\
iscas89-s1488 & 7 & 3.37 & 3 & 53 & 779 & 463 & 174.40 & 315.73 & 0.03 \\
iscas89-s1494 & 7 & 3.37 & 3 & 56 & 796 & 473 & 174.40 & 316.10 & 0.03 \\
iscas89-s15850 & 4 & 2.47 & 4 & 25 & 4004 & 3247 & 418.71 & 1296.03 & 0.05 \\
iscas89-s27 & 1 & 1.78 & 1 & 3 & 8 & 9 & 84.46 & 84.46 & 0.02 \\
iscas89-s298 & 3 & 2.85 & 2 & 11 & 131 & 92 & 94.33 & 94.33 & 0.02 \\
iscas89-s344 & 3 & 2.44 & 2 & 9 & 122 & 100 & 93.55 & 93.55 & 0.02 \\
iscas89-s349 & 3 & 2.49 & 2 & 9 & 127 & 102 & 94.15 & 94.15 & 0.02 \\
iscas89-s35932 & 2 & 2.55 & 2 & 1440 & 15961 & 12515 & 1496.98 & 5156.41 & 0.13 \\
iscas89-s382 & 4 & 2.90 & 2 & 18 & 168 & 116 & 105.42 & 105.42 & 0.02 \\
iscas89-s38417 & 6 & 2.24 & 4 & 39 & 10635 & 9500 & 1488.70 & 5017.87 & 0.17 \\
iscas89-s38584 & 7 & 2.74 & 4 & 54 & 12573 & 9193 & 1503.33 & 5036.81 & 0.28 \\
iscas89-s386 & 4 & 3.51 & 3 & 23 & 200 & 114 & 106.01 & 106.01 & 0.03 \\
iscas89-s400 & 4 & 3.01 & 2 & 19 & 182 & 121 & 105.44 & 105.44 & 0.03 \\
iscas89-s444 & 4 & 3.07 & 2 & 19 & 206 & 134 & 105.50 & 105.50 & 0.04 \\
iscas89-s510 & 4 & 2.92 & 2 & 12 & 251 & 172 & 105.32 & 105.32 & 0.03 \\
iscas89-s526 & 4 & 3.38 & 3 & 12 & 270 & 160 & 105.60 & 105.60 & 0.02 \\
iscas89-s526n & 4 & 3.37 & 3 & 12 & 268 & 159 & 105.61 & 105.61 & 0.03 \\
iscas89-s5378 & 5 & 2.32 & 3 & 10 & 1639 & 1411 & 257.70 & 633.07 & 0.06 \\
iscas89-s641 & 4 & 2.88 & 3 & 12 & 144 & 100 & 93.57 & 93.57 & 0.04 \\
iscas89-s713 & 4 & 2.63 & 3 & 12 & 180 & 137 & 105.07 & 105.07 & 0.03 \\
iscas89-s820 & 9 & 4.02 & 3 & 48 & 480 & 239 & 129.70 & 160.27 & 0.04 \\
iscas89-s832 & 9 & 4.07 & 3 & 49 & 498 & 245 & 129.52 & 161.36 & 0.04 \\
iscas89-s9234 & 4 & 2.39 & 4 & 18 & 2370 & 1985 & 419.55 & 1243.79 & 0.06 \\
iscas89-s953 & 3 & 2.73 & 2 & 12 & 454 & 332 & 127.39 & 160.63 & 0.03 \\
jazz & 30 & 27.70 & 29 & 100 & 2742 & 198 & 141.45 & 211.72 & 0.05 \\
karate & 4 & 4.59 & 4 & 17 & 78 & 34 & 88.95 & 88.95 & 0.03 \\
lederberg & 47 & 9.98 & 15 & 1103 & 41532 & 8324 & 1852.88 & 5968.18 & 1.93 \\
lesmiserables & 9 & 6.60 & 9 & 36 & 254 & 77 & 94.71 & 94.71 & 0.04 \\
link-pedigree & 2 & 2.51 & 2 & 14 & 1125 & 898 & 258.84 & 615.70 & 0.03 \\
linux & 106 & 13.83 & 23 & 9338 & 213217 & 30834 & 8177.22 & 25761.40 & 24.34 \\
livemocha & 610 & 42.13 & 92 & 2980 & 2193083 & 104103 & 49622.93 & 163105.27 & 4456.76 \\
loc-brightkite\_edges & 85 & 7.35 & 52 & 1134 & 214078 & 58228 & 13050.88 & 43914.91 & 18.08 \\
location & 16 & 2.61 & 5 & 12189 & 293697 & 225486 & 23410.76 & 84379.95 & 21.74 \\
mag\_geology\_coauthor & 31 & 3.12 & 13 & 1153 & 4448428 & 2852295 & 369765.78 & 1331825.50 & 5345.90 \\
marvel & 58 & 9.95 & 18 & 1625 & 96662 & 19428 & 3554.43 & 12827.92 & 5.46 \\
mg\_casino & 9 & 5.98 & 9 & 94 & 326 & 109 & 96.15 & 96.15 & 0.03 \\
mg\_forrestgump & 8 & 5.77 & 8 & 89 & 271 & 94 & 95.35 & 95.35 & 0.03 \\
mg\_godfatherII & 8 & 5.62 & 8 & 34 & 219 & 78 & 94.38 & 94.38 & 0.02 \\
mg\_watchmen & 7 & 5.29 & 7 & 33 & 201 & 76 & 94.48 & 94.48 & 0.03 \\
minnesota & 3 & 2.50 & 2 & 5 & 3303 & 2642 & 431.87 & 1257.38 & 0.04 \\
moreno\_health & 12 & 8.24 & 7 & 27 & 10455 & 2539 & 484.67 & 1525.81 & 0.12 \\
mousebrain & 141 & 151.07 & 111 & 205 & 16089 & 213 & 443.32 & 882.01 & 0.20 \\
movielens\_1m & 554 & 205.26 & 131 & 3428 & 1000209 & 9746 & 22602.53 & 69027.36 & 777.59 \\
movies & 5 & 3.80 & 3 & 19 & 192 & 101 & 94.19 & 94.19 & 0.03 \\
muenchen-bahn & 3 & 2.59 & 2 & 13 & 578 & 447 & 126.32 & 172.26 & 0.03 \\
munin & 3 & 2.11 & 3 & 66 & 1397 & 1324 & 258.60 & 631.20 & 0.04 \\
netscience & 19 & 3.75 & 19 & 34 & 2742 & 1461 & 263.98 & 659.91 & 0.11 \\
offshore & 20 & 3.63 & 13 & 37336 & 505965 & 278877 & 45987.69 & 164611.63 & 41.04 \\
openflights & 52 & 10.67 & 28 & 242 & 15677 & 2939 & 588.65 & 1808.73 & 0.36 \\
p2p-Gnutella04 & 23 & 7.35 & 7 & 103 & 39994 & 10876 & 1691.07 & 6104.80 & 1.18 \\
panama & 62 & 2.52 & 62 & 7015 & 702437 & 556686 & 90229.39 & 321508.06 & 191.64 \\
paradise & 55 & 2.93 & 23 & 35359 & 794545 & 542102 & 92879.70 & 324180.06 & 220.41 \\
photoviz\_dynamic & 7 & 3.24 & 4 & 29 & 610 & 376 & 127.98 & 165.08 & 0.02 \\
pigs & 3 & 2.41 & 2 & 39 & 592 & 492 & 171.13 & 310.38 & 0.05 \\
polblogs & 72 & 27.31 & 36 & 351 & 16715 & 1224 & 470.51 & 1401.45 & 0.38 \\
polbooks & 9 & 8.40 & 6 & 25 & 441 & 105 & 97.88 & 97.88 & 0.05 \\
pollination-carlinville & 53 & 20.34 & 18 & 157 & 15255 & 1500 & 453.09 & 1365.70 & 0.58 \\
pollination-daphni & 26 & 7.36 & 9 & 124 & 2933 & 797 & 198.24 & 419.46 & 0.08 \\
pollination-tenerife & 6 & 3.79 & 4 & 17 & 129 & 68 & 94.84 & 94.84 & 0.04 \\
pollination-uk & 76 & 33.97 & 35 & 256 & 16712 & 984 & 460.78 & 1431.23 & 0.83 \\
ratbrain & 78 & 91.57 & 67 & 497 & 23030 & 503 & 550.80 & 1234.35 & 0.27 \\
reactome & 184 & 46.64 & 62 & 855 & 147547 & 6327 & 3316.78 & 9729.96 & 7.05 \\
residence\_hall & 21 & 16.95 & 11 & 56 & 1839 & 217 & 127.13 & 166.53 & 0.04 \\
rhesusbrain & 37 & 25.24 & 19 & 111 & 3054 & 242 & 160.76 & 281.81 & 0.10 \\
roget-thesaurus & 11 & 7.22 & 6 & 28 & 3648 & 1010 & 281.48 & 684.80 & 0.04 \\
seventh-graders & 16 & 17.24 & 13 & 28 & 250 & 29 & 90.82 & 90.82 & 0.03 \\
slashdot\_threads & 74 & 4.60 & 13 & 2915 & 117378 & 51083 & 6330.25 & 22970.25 & 10.16 \\
soc-Epinions1 & 268 & 10.69 & 67 & 3044 & 405740 & 75879 & 16119.82 & 53521.95 & 104.16 \\
soc-Slashdot0811 & 232 & 12.13 & 54 & 2539 & 469180 & 77360 & 16037.11 & 57199.10 & 209.41 \\
soc-advogato & 86 & 15.26 & 25 & 807 & 39432 & 5167 & 1200.26 & 4113.99 & 2.56 \\
soc-gplus & 38 & 3.32 & 12 & 2761 & 39194 & 23628 & 3099.64 & 10679.76 & 1.26 \\
soc-hamsterster & 51 & 13.71 & 24 & 273 & 16630 & 2426 & 609.35 & 1860.52 & 0.68 \\
soc-wiki-Vote & 16 & 6.56 & 9 & 102 & 2914 & 889 & 194.76 & 415.82 & 0.07 \\
sp\_data\_school\_day\_2 & 57 & 46.55 & 33 & 88 & 5539 & 238 & 200.84 & 429.13 & 0.11 \\
teams & 127 & 2.92 & 9 & 2671 & 1366466 & 935591 & 180105.19 & 648392.60 & 1031.76 \\
train\_bombing & 10 & 7.59 & 10 & 29 & 243 & 64 & 96.34 & 96.34 & 0.02 \\
tv\_tropes & 655 & 42.50 & 115 & 12400 & 3232134 & 152093 & 80649.22 & 261756.61 & 6861.11 \\
twittercrawl & 237 & 84.70 & 131 & 1084 & 154824 & 3656 & 3414.48 & 10744.15 & 60.97 \\
ukroad & 3 & 2.53 & 3 & 5 & 15641 & 12378 & 1392.84 & 5052.68 & 0.20 \\
unicode\_languages & 7 & 2.89 & 4 & 141 & 1255 & 868 & 173.08 & 332.53 & 0.03 \\
wafa-ceos & 7 & 7.15 & 5 & 22 & 93 & 26 & 86.51 & 86.51 & 0.04 \\
wafa-eies & 27 & 28.98 & 24 & 44 & 652 & 45 & 97.84 & 97.84 & 0.03 \\
wafa-hightech & 13 & 15.14 & 12 & 20 & 159 & 21 & 87.76 & 87.76 & 0.02 \\
wafa-padgett & 3 & 3.60 & 3 & 8 & 27 & 15 & 85.95 & 85.95 & 0.02 \\
web-EPA & 16 & 4.17 & 6 & 175 & 8909 & 4271 & 802.68 & 2611.49 & 0.36 \\
web-california & 26 & 5.17 & 11 & 199 & 15969 & 6175 & 859.52 & 2909.39 & 0.52 \\
web-google & 17 & 4.27 & 17 & 59 & 2773 & 1299 & 264.85 & 665.56 & 0.05 \\
wiki-vote & 162 & 28.32 & 53 & 1065 & 100762 & 7115 & 2226.58 & 7802.97 & 26.17 \\
wikipedia-norm & 59 & 16.34 & 22 & 455 & 15372 & 1881 & 594.99 & 1764.65 & 0.53 \\
win95pts & 3 & 2.26 & 2 & 9 & 112 & 99 & 94.17 & 94.17 & 0.02 \\
windsurfers & 15 & 15.63 & 11 & 31 & 336 & 43 & 92.03 & 92.03 & 0.03 \\
word\_adjacencies & 11 & 7.59 & 6 & 49 & 425 & 112 & 99.66 & 99.66 & 0.04 \\
zewail & 55 & 16.29 & 18 & 331 & 54182 & 6651 & 1441.94 & 4931.46 & 2.87 \\
\hline
\end{longtable}

